DNN-Chip Predictor: An Analytical Performance Predictor for DNN Accelerators with Various Dataflows and Hardware Architectures

The recent breakthroughs in deep neural networks (DNNs) have spurred a tremendously increased demand for DNN accelerators. However, designing DNN accelerators is non-trivial as it often takes months/years and requires cross-disciplinary knowledge. To enable fast and effective DNN accelerator development, we propose DNN-Chip Predictor, an analytical performance predictor which can accurately predict DNN accelerators' energy, throughput, and latency prior to their actual implementation. Our Predictor features two highlights: (1) its analytical performance formulation of DNN ASIC/FPGA accelerators facilitates fast design space exploration and optimization; and (2) it supports DNN accelerators with different algorithm-to-hardware mapping methods (i.e., dataflows) and hardware architectures. Experiment results based on 2 DNN models and 3 different ASIC/FPGA implementations show that our DNN-Chip Predictor's predicted performance differs from those of chip measurements of FPGA/ASIC implementation by no more than 17.66% when using different DNN models, hardware architectures, and dataflows. We will release code upon acceptance.

==> tex/3-Proposed-backup.tex <==
\section{The Proposed \textit{DNN-Chip Predictor}}\label{sec:proposed}
%This section describes the \textit{DNN-Chip Predictor}'s features and its simulation methodologies. 

\subsection{One-For-All Graph-based Accelerator Description}\label{subsec:graph}
For reducing the prediction error, it is critical that the design space can be precisely and concisely described, e.g., the different levels of accelerator design optimization (including architecture level, IP level, and algorithm-to-hardware mapping level) are considered. To this end, we adopt an object-oriented directed graph for the DNN accelerator design space description. 
Specifically, a basic directed graph is first constructed based on the PE (processing engine) array architecture, memory design, and DNN-to-hardware mapping methods, where each node in the graph denotes a computation IP, data path IP, or memory IP and each directed edge denotes an inter-connection between nodes whose direction is determined by the direction of data movement. 
Proper attributes as shown in Table~\ref{tab:nodes_edges}, such as data type, bandwidth, and frequency, are then assigned to the nodes and edges of the directed graph in an object-oriented manner. Fig.~\ref{fig:template} shows the graph-based description of systolic architecture on ASIC and a commonly-used spatial architecture on FPGA.  
A state machine reflects mapping is employed in each IP to simulate, analyze, and record switching in the graph-based description. A state machine can be treated as a subset of loops in the for-loop description as in~\cite{parashar2019timeloop,chen2018eyerissv2} which is related to this IP. A central controller stores the overall data scheduling in nested for-loop format.  
%\todor{For coarse-grained and fine-grained mode, the switching requirement is different that}.

\begin{table}[h!]
\vspace{-0em}
\caption{A summary of attributes for graph nodes and edges in the graph-based description.}
%common attributes among the three: and single attributes
\vspace{-1em}
\def\arraystretch{1.2}
\centering
%\fontsize{7.5}{9}\selectfont
\scriptsize
\tiny
\begin{tabular}{|c|c|c|}
\hline
{\textbf{Compo.$^a$}} & {\textbf{Hardware meaning}} & {\textbf{Attributes}} \\
\hline
\multirow{3}{*}{Node} & {Memory IPs} & {Impl. Freq. Vol. Prec. Dt. StM.$^b$}\\
\cline{2-3}
 & {Computation IPs} & {Impl. Freq. Prec. StM.}\\
\cline{2-3}
 & {Data Path IPs} & {Impl. Freq. Vol. Bw. Prec. Dt. StM.$^c$}\\
\cline{2-3}
%  & {Controller IPs} & {Overhead $^e$}\\
\hline
{Edge} & {IP inter-connections} & {Start. End $^d$}\\
\hline
\end{tabular}
%\centering
\begin{tablenotes}
\item{$^a$ Compo.: Graph components including nodes and directed edges.}\\
\item{$^b$ Impl.: implementation, e.g. 14nm DRAM, 65nm SRAM, DSP48E, axi-bus, sync FIFO, etc}\\
\item{$\quad$ Freq.: clock frequency (MHz), Vol.: Volume/Capacity (bits) Prec.: bit precision}\\
\item{$\quad$ Dt.: data type including weight, input activations, partial sums.}\\
\item{$\quad$ StM.: state machine storing all the states (needed input, generated output) through the whole execution process.}\\
\item{$^c$ Bw.: port width/bus width. $^e$ Overhead: energy/latency overhead.}\\
\item{$^d$ Start. \& End: the start and ending node for the directed edge}.\\
\end{tablenotes}
\vspace{-0pt}
% \caption{A summary of attributes for the nodes and edges in the graph-based description.}
\label{tab:nodes_edges}
%\vspace{-0pt}
\vspace{-1.3em}
\end{table}

\begin{figure}[h]
    \centerline{\includegraphics[width=1\linewidth]{fig/two_template.pdf}}
    \vspace{-1em}
    \caption{Two architecture examples (a) systolic architecture on ASIC and (b) spatial architecture on FPGA.}
    \label{fig:template}
\end{figure}

\subsection{Coarse-grained \textit{DNN-Chip Predictor}}\label{subsec:coarse}
%This subsection introduces our proposed analytical-models for use in the \textit{DNN-Chip Predictor}'s coarse-grained mode. These models are based the attributes of each IP and ignore the inter-IP pipeline dependence for fast prediction. 
From a high-level view, \textit{DNN-Chip Predictor}'s coarse-grained mode depends on the nested for-loop and the attributes of each IP and ignore the inter-IP pipeline dependence for fast prediction. 
\textbf{Energy Model:} the energy of DNN accelerators include both computational and data movement costs, both of which equal the product between the total number of operations (e.g., computation or data access) and the unit energy of the operations. 
While the total number of computations of computation IP is easily obtained from the state machine, the key challenge is to obtain the total number of accesses to various memory IPs for varied data types (e.g., weights, inputs, or activations). Coarse-grained prediction uses the overall nested for-loop to analytically formulate such accesses for fast prediction. 
We propose that the total number of those accesses can be calculated as the product between the data volume involved in each memory refresh and the total number of such refreshes for the corresponding memory IP. 
Furthermore, to obtain the involved data volume and total number of memory refreshes, we propose an intuitive methodology: we first \ul{\textbf{(i)}} choose a refresh location within the nested for-loop description, which is determined by the given DNN-to-hardware mapping methods; \ul{\textbf{(ii)}} the total number of the memory refreshes is equal to the product of all the loop bounds in the for-loops \textbf{below} the refresh location for the particular type of data; and \ul{\textbf{(iii)}} the total data volume corresponding to the refresh is equal to the product of all the loop bounds in the for-loops \textbf{above} the refresh location and associated with this data type.
%While the unit energy is obtained from single-IP test experiment repeated by multiple times and the total number of computations of computation IP is easily gotten from the state machine, the key challenge is to obtain the total number of accesses to various memory IPs for varied data types (e.g., weights, inputs, or activations). We further divide the memory IP accesses into two types according to the edge in graph: (1) the edges whose start point is the memory IP and the corresponding memory accesses is from the memory IP to the memory data consuming IP and (2) the edges whose end point is the memory IP and the corresponding memory access is from the memory data providing IP to memory IP. 
%We propose that the total number of those accesses can be calculated as the product between the data volume involved in each memory refresh and the total number of such refreshes for the corresponding memory IP. 
%Further, to obtain the involved data volume and total number of memory refreshes, we propose an intuitive methodology: we first \ul{\textbf{(i)}} choose a refresh location within the state machine, which is determined by the given algorithm-to-hardware mapping methods; \ul{\textbf{(ii)}} the total number of the memory refreshes is equal to the product of all the switches from that refresh location state; and \ul{\textbf{(iii)}} the total data volume corresponding to the refresh is equal to data associated in this state.
\textbf{Latency Model:} we simply add up all the IPs' delay of the longest path in graph which can be analytically modelled. \textbf{Resource Model:} the total resource is estimated as the sum of all the resources in the accelerator design. 

%Thrust 1's IP Creator which characterizes technology based IP performance, the key challenge is to obtain the total number of accesses to various memory hierarchies for varied data types (e.g., weights, inputs, or activations) when using different AI algorithms, hardware configurations, and algorithm-to-hardware mapping methods. 
%We propose that the total number of such accesses can be calculated as the product between the data volume involved in each memory refresh and the total number of such refreshes for the corresponding memory. 
%Furthermore, to obtain the involved data volume and total number of memory refreshes, \textbf{we propose an intuitive methodology}: we first \ul{\textbf{(i)}} choose a refresh location within the nested for-loop description, which is determined by the given algorithm-to-hardware mapping methods; \ul{\textbf{(ii)}} the total number of the memory refreshes is equal to the product of all the loop bounds in the for-loops \textbf{below} the refresh location for the particular type of data; and \ul{\textbf{(iii)}} the total data volume corresponding to the refresh is equal to the product of all the loop bounds in the for-loops \textbf{above} the refresh location and associated with this data type. 
%Similarly, the latency, throughput, and area of AI accelerators can be analytically modelled.


\subsection{Fine-grained \textit{DNN-Chip Predictor}}\label{subsec:fine}
In this subsection, we describe the proposed fine-grained \textit{DNN-Chip Predictor}, which features the graph-based design space description and the employment of a state machine to characterize the inter-IP pipeline dependence given that pipelining is a fundamental technique to improve chip throughput and performance. 
Compared with coarse-grained mode, fine-grained prediction is simulation-based. In particular, in each state of the state machine, the addresses corresponding to each IP's required inputs are generated; the states of all the IPs in the graph are updated as follows: each IP will jump to the next state (being busy) if it is idle and all its needed inputs can be found from its preceding IPs in the graph. 
\textbf{Latency Model:} the latency calculation uses the run-time simulation based on the state switching of the IPs. 
Fig.~\ref{fig:toy1} and Fig.~\ref{fig:toy2} show two toy examples where the fine-grained mode of \textit{DNN-Chip Predictor} can enable inter-IP pipeline to accurately estimate the latency.  
In Fig.~\ref{fig:toy1}, the systolic array with 9 computation IPs processes the task of matrix-matrix multiplication. The critical path in coarse-grained mode is as in Fig.~\ref{fig:toy1} (b) whose latency is 15. In fine-grained mode, inter-IP pipeline is enabled where the switch from one state to the next state depends on the availability of required data as shown in Fig.~\ref{fig:toy1} (c) resulting in 7 latency. Although coarse-grained mode is not accurate as fine-grained mode, the trend are correct, e.g., scaling up of IPs will result in a shorter latency, which is acceptable considering its speed.   
Fig.~\ref{fig:toy2} is a toy example of one data path IP and one computation IP in graph. The task is initially divided into 4 tiles. In fine-grained mode, if there is enough resource, pipeline is inserted as in Fig.~\ref{fig:toy2} (c) to achieve a smaller latency compared to Fig.~\ref{fig:toy2} (c). \textbf{Resource Model:} as shown in Fig.~\ref{fig:toy2} (c), some pipeline design requires more resource than none-pipeline design. Fine-grained \textit{DNN-Chip Predictor} considers the resource overhead which is critical for the estimation of resource-configurable accelerator design. 

\begin{figure}[h]
    \centerline{\includegraphics[width=0.8\linewidth]{fig/systolic.pdf}}
    \caption{A toy example of systolic array: (a) a task of matrix-matrix multiplication, (b) a systolic array with 9 computation IPs, and (c) fine-grained latency estimation.}
    \label{fig:toy1}
\end{figure}

\begin{figure}[h]
    \centerline{\includegraphics[width=0.8\linewidth]{fig/toy2_new.pdf}}
    \caption{A toy example of inter-IP pipeline:
    (a) a simple architecture with two IPs, i.e., one data path IP and one computation IP, pipeline unabled (b) and enabled latency estimation (c), and a optimized pipeline design (d).}
    \label{fig:toy2}
\end{figure}

\subsection{Bottleneck Analyzer}\label{subsec:bottlenech}
The proposed \textit{DNN-Chip Predictor} outputs the bottleneck IPs to enable design optimization when using simulation-based fine-grained estimation. Take Fig.~\ref{fig:toy2} (d) as an example, the bottleneck IPs are recorded and then optimized via tiling and reordering. This optimized pipeline design has a smaller pipeline stage and the resulting latency and idle cycles are reduced. 





==> tex/3-Proposed.tex <==
\vspace{-1.2em}
\section{The Proposed \textit{DNN-Chip Predictor}}\label{sec:proposed}
    \vspace{-1em}
\subsection{Overview}
    \vspace{-0.7em}
\label{subsec:coarse_pred}
% \textbf{Overview of the proposed \textit{DNN-Chip Predictor}}. 
% The proposed \textit{DNN-Chip Predictor} can estimate the energy, latency and resource consumption of a DNN accelerator given the hardware design including architecture choices, IP design and hardware mapping as shown in FIg.~\ref{fig:chip_predictor}. 

As shown in Fig.~\ref{fig:chip_predictor}, the proposed \textit{DNN-Chip Predictor} accepts DNN models, hardware architectures, hardware mapping, and IP design, and then outputs the estimated energy consumption, latency, and resource consumption when executing the DNN in a target accelerator defined by the specified hardware architecture and mapping choices. To capture the large search space and consider all the design levels (including architecture level, IP level, and hardware mapping level), we construct a graph-based description (Section \ref{sec:graph}) for use as the input of \textit{DNN-Chip Predictor}.
Our \textit{DNN-Chip Predictor} features a mixed-granularity prediction, i.e., including 1) a coarse-grained mode (Section \ref{subsec:coarse}) that can quickly provide performance estimation and identify the critical paths when the inter-IP pipeline is not considered, which can be used for early-stage architecture and IP selection; and 2) a fine-grained mode (Section \ref{subsec:fine}) that can perform accurate performance prediction considering inter-IP pipeline based on run-time simulations.

% Overall, the proposed \textit{DNN-Chip Predictor} features three characteristics: 1) it supports performance prediction of arbitrary graph-defined architectures and platforms/DNNs; and it includes 2) a coarse-grained mode that facilitates the \textit{Chip Builder}'s early-stage architecture-IP co-exploration which requires fast elimination of infeasible designs; and 3) a fine-grained mode for supporting the IP-pipeline co-exploration which requires accurate prediction of pipelined latency, and correct prediction of the system bottleneck. 

\begin{figure}[h]
    \vspace{-0.9em}
    \centerline{\includegraphics[width=0.9\linewidth]{fig/Predictor.pdf}}
    \vspace{-0.8em}
    \caption{A high-level view of the \textit{DNN-Chip Predictor}.}
     \vspace{-1.3em}
    \label{fig:chip_predictor}
\end{figure}


    \vspace{-1.3em}
\subsection{One-For-All Graph-based Design Space Description}
    \vspace{-0.7em}
\label{sec:graph}
For reducing the prediction error, it is critical that the design space can be precisely and concisely described, e.g., the different levels of accelerator design optimization (including architecture level, IP level, and algorithm-to-hardware mapping level) are captured. To this end, we adopt an object-oriented directed graph for the DNN accelerator design space description. 
Specifically, a basic directed graph is first constructed based on the PE (processing engine) array architecture, memory design, and DNN-to-hardware mapping methods, where each node in the graph denotes a computation，data path, or memory IP while each directed edge denotes an inter-connection between nodes whose direction is determined by the actual data movement direction. 
Considered attributes (see Table~\ref{tab:nodes_edges}), such as data type, bandwidth, and frequency, are then assigned to the nodes and edges of the directed graph in an object-oriented manner. 
% Fig.~\ref{fig:template} shows the graph-based description of systolic architecture on ASIC and a commonly-used spatial architecture on FPGA.
A state machine reflecting mapping methods is employed in each IP to simulate, analyze, and record switching activities in the graph-based description, which can be treated as a subset of loops, that are related to the corresponding IP, in the for-loop description as in~\cite{parashar2019timeloop,chen2018eyerissv2}. A central controller stores the overall data scheduling in a nested for-loop format.  
%\todor{For coarse-grained and fine-grained mode, the switching requirement is different that}.

% \begin{table}[h!]
% \vspace{-0.8em}
% \caption{A summary of attributes for graph nodes and edges.}
% %common attributes among the three: and single attributes
% \vspace{-1em}
% \def\arraystretch{1.2}
% \centering
% %\fontsize{7.5}{9}\selectfont
% \scriptsize
% \tiny
% \begin{tabular}{|c|c|c|}
% \hline
% {\textbf{Graph components}} & {\textbf{Hardware meaning}} & {\textbf{Attributes}} \\
% \hline
% \multirow{3}{*}{Node} & {Memory IPs} & {(Implementation, Freq., Vol., Prec., Dt., StM.)$^a$}\\
% \cline{2-3}
%  & {Computation IPs} & {(Implementation, Freq., Prec., StM.)}\\
% \cline{2-3}
%  & {Data Path IPs} & {(Implementation Freq., Vol., Bw., Prec., Dt., StM.)$^b$}\\
% \cline{2-3}
% %  & {Controller IPs} & {Overhead $^e$}\\
% \hline
% {Edge} & {IP inter-connections} & {(Start, End) $^c$}\\
% \hline
% \end{tabular}
% %\centering
% \begin{tablenotes}
% % \item{$^a$ Compo.: Graph components including nodes and directed edges.}\\
% \item{$^a$ Implementation, e.g. 14nm DRAM, 65nm SRAM, DSP48E, axi-bus, sync FIFO, etc}\\
% \item{$\quad$ Freq.: clock frequency (MHz), Vol.: Volume/Capacity (bits), Prec.: bit precision}\\
% \item{$\quad$ Dt.: data type including weight, input activations, partial sums.}\\
% \item{$\quad$ StM.: state machine storing all the states (needed input, generated output) through the whole execution process.}\\
% \item{$^b$ Bw.: port width/bus width.}\\
% \item{$^c$ Start. \& End: the start and ending node for the directed edge}.\\
% \end{tablenotes}
% \vspace{-0pt}
% % \caption{A summary of attributes for the nodes and edges in the graph-based description.}
% \label{tab:nodes_edges}
% %\vspace{-0pt}
% \vspace{-1.5em}
% \end{table}

\begin{table}[h!]
\vspace{-0.8em}
\caption{A summary of attributes for graph nodes and edges.}
%common attributes among the three: and single attributes
\vspace{-1em}
\def\arraystretch{1.2}
\centering
%\fontsize{7.5}{9}\selectfont
\scriptsize
\tiny
\begin{tabular}{|c|c|c|}
\hline
{\textbf{Graph components}} & {\textbf{Hardware meaning}} & {\textbf{Attributes}} \\
\hline
\multirow{2}{*}{Node} & {Memory IPs} & {(Implementation, Freq., Vol., Prec., Dt., StM.)$^a$}\\
\cline{2-3}
 & {Computation IPs} & {(Implementation, Freq., Prec., StM.)}\\
\cline{2-3}
\hline
{Edge} & {Data Path IPs} & {(Implementation, Freq., Vol., Prec., Dt., StM., Bw., Start, End) $^b$}\\
\hline
\end{tabular}
%\centering
\begin{tablenotes}
% \item{$^a$ Compo.: Graph components including nodes and directed edges.}\\
\item{$^a$ Implementation, e.g. 14nm DRAM, 65nm SRAM, DSP48E, axi-bus, sync FIFO, etc}\\
\item{$\quad$ Freq.: clock frequency (MHz), Vol.: Volume/Capacity (bits), Prec.: bit precision}\\
\item{$\quad$ Dt.: data type including weight, input activations, partial sums.}\\
\item{$\quad$ StM.: state machine storing all the states (needed input, generated output) through the whole execution process.}\\
\item{$^b$ Bw.: port width/bus width.}\\
\item{$\quad$ Start. \& End: the start and ending node for the directed edge}.\\
\end{tablenotes}
\vspace{-0pt}
% \caption{A summary of attributes for the nodes and edges in the graph-based description.}
\label{tab:nodes_edges}
%\vspace{-0pt}
\vspace{-1.5em}
\end{table}

\begin{figure}[h]
\vspace{-1em}
    \centerline{\includegraphics[width=1\linewidth]{fig/two_template.pdf}}
    \vspace{-1em}
    \caption{Two architecture examples: (a) a systolic architecture and (b) a spatial architecture.}
    \label{fig:template}
     \vspace{-1.7em}
\end{figure}

    \vspace{-0.7em}
\subsection{Coarse-grained \textit{DNN-Chip Predictor}}\label{subsec:coarse}
    \vspace{-0.7em}
%This subsection introduces our proposed analytical-models for use in the \textit{DNN-Chip Predictor}'s coarse-grained mode. These models are based the attributes of each IP and ignore the inter-IP pipeline dependence for fast prediction. 
\textit{DNN-Chip Predictor}'s coarse-grained mode adopts a nested for-loop description \cite{eyeriss} and ignore the inter-IP pipeline dependence for fast prediction. 
\textbf{Energy Model:} the energy of DNN accelerators include both computational and data movement costs, both of which are equal to the product between the total number of operations (e.g., computation or data access) and the unit energy of the operations. 
While the total number of computations of computation IPs can be easily obtained from the state machine, the key challenge is to obtain the total number of accesses to various memory IPs for varied data types (e.g., weights, inputs, or activations), which is analytically formulated based on a nested for-loop description in our coarse-grained prediction for fast prediction. 
We found that \textit{the total number of memory accesses can be calculated as the product between the data volume involved in each memory refresh and the total number of such refreshes for the corresponding memory IP}. 
Furthermore, to obtain the involved data volume and total number of memory refreshes, we propose \textit{an intuitive methodology}: 
% we first \ul{\textit{(i)}} choose a refresh location within the nested for-loop description, which is determined by the given DNN-to-hardware mapping methods; \ul{\textit{(ii)}} the total number of the memory refreshes is equal to the product of all the loop bounds in the for-loops \textbfit total data volume corresponding to the refresh is equal to the product of allithe loop bounds in the for-loops \textit{above} the refresh location and associated with this data type.
we first \ul{\textit{(i)}} choose a refresh location within the nested for-loop description depending on the given algorithm-to-hardware mapping methods; \ul{\textit{(ii)}} the total number of memory refreshes is equal to the product of all the loop bounds in the for-loops \textit{above} the refresh location for the particular type of data; and \ul{\textit{(iii)}} the total data volume corresponding to the refresh is equal to the product of all the loop bounds in the for-loops \textit{below} the refresh location and associated with the corresponding type of data.
\textbf{Latency Model:} the coarse-grained latency is defined as the latency of the longest path in the graph which can also be analytically formulated. 

  \vspace{-1.5em}
\subsection{Fine-grained \textit{DNN-Chip Predictor}}\label{subsec:fine}
  \vspace{-0.7em}
Given that pipelining is a fundamental technique determining processing throughput and performance, our proposed fine-grained \textit{DNN-Chip Predictor} features a graph-based design space description and a state machine that characterizes the inter-IP pipeline dependency. 
Built on top of the coarse-grained mode, the fine-grained prediction adds simulation-based characterization of inter-IP pipeline dependency. In particular, in each state of the state machine, the addresses corresponding to each IP's required inputs are generated; the states of all the IPs in the graph are updated as follows: each IP will jump to the next state (being busy) if it is idle and all its needed inputs can be found from its preceding IPs in the graph. 
\textbf{Latency Model:} the latency calculation makes use of run-time simulations based on the IPs' state switching activities. 
Fig.~\ref{fig:toy1} and Fig.~\ref{fig:toy2} are two toy examples showing the fine-grained mode of \textit{DNN-Chip Predictor} can capture inter-IP pipeline to more accurately estimate the latency.  
In Fig.~\ref{fig:toy1}, the systolic array with 9 computation IPs processes a task of matrix-matrix multiplications. The critical path in the coarse-grained mode shown in Fig.~\ref{fig:toy1} (b) has 15 units of latency. In the fine-grained mode, inter-IP pipeline is enabled where the switching from one state to the next state depends on the availability of required data as shown in Fig.~\ref{fig:toy1} (c) resulting in 7 units of latency. Although the coarse-grained mode is not as accurate as the fine-grained one, the ranking of the predicted performance is correct, e.g., scaling up of IPs will result in a shorter latency, and thus is sufficiently effective for ruling out inappropriate design choices.   
Fig.~\ref{fig:toy2} is a toy example of one data path and computation IPs in the graph performing a task that is initially divided into 4 tiles. In the fine-grained mode, if there is enough resource, pipeline can be inserted as in Fig.~\ref{fig:toy2} (c) to achieve a smaller latency compared to Fig.~\ref{fig:toy2} (b). \textbf{Resource Model:} as shown in Fig.~\ref{fig:toy2} (c), some pipeline designs require more resource than a no-pipeline design. Fine-grained \textit{DNN-Chip Predictor} considers such resource overheads which is critical for estimating resource-configurable accelerators. 

\begin{figure}[h]
    \vspace{-1em}
    \centerline{\includegraphics[width=0.7\linewidth]{fig/systolic.pdf}}
        \vspace{-0.7em}
    \caption{An example showing: (a) matrix-matrix multiplication, and (b) coarse-grained and (c) fine-grained latency estimation.}
        \vspace{-0.7em}
    \label{fig:toy1}
\end{figure}

\begin{figure}[h]
    \vspace{-1.1em}
    \centerline{\includegraphics[width=0.7\linewidth]{fig/toy2.pdf}}
        \vspace{-0.7em}
    \caption{An example of inter-IP pipeline:
    (a) a simple architecture with two IPs, i.e., one data path IP and one computation IP, (b) coarse-grained and fine-grained (c) latency estimation.}
        \vspace{-1em}
    \label{fig:toy2}
\end{figure}

%         \vspace{-1.3em}
% \subsection{Bottleneck Analyzer}\label{subsec:bottlenech}
% The proposed \textit{DNN-Chip Predictor} outputs the bottleneck IPs to enable design optimization when using simulation-based fine-grained estimation. Take Fig.~\ref{fig:toy2} (d) as an example, the bottleneck IPs are recorded and then optimized via tiling and reordering. This optimized pipeline design has a smaller pipeline stage and the resulting latency and idle cycles are reduced. 




==> tex/4-Experiment.tex <==
\vspace{-1.2em}
\section{Experiment Results}
\vspace{-1em}
%In this section, we validate the proposed \textit{DNN-Chip Predictor} by comparing its predicted performance with real-device measured and reported state-of-the-art accelerators in terms of energy consumption, latency, and resource consumption.

\textbf{Methodology and Setup.} Experiment settings are listed in Table~\ref{tab:val_setting}.
% including the platforms/accelerators, performance metrics, DNN models, methods to obtain the unit parameters, employed precision for the weights and activations, and frequency of the corresponding computation core. 
We validate the \textit{DNN-Chip Predictor} by comparing its predicted performance with 1) actual device measurements on \ul{edge devices} (edge FPGA~\cite{ultra96}, edge TPU~\cite{edgetpu}, edge GPU ~\cite{edgegpu}) and 2) that of \ul{published ASIC accelerators}~\cite{eyeriss,du2015shidiannao}) under the same settings. For edge devices, we consider 15 representative DNN models, including 10 variants (M1-M10) of SkyNet in \cite{zhang2019skynet}, and 5 variants (M11-M15) of MobileNetV2 in ~\cite{mobilenetv2}; for the ASIC  accelerators, we use the same DNN models and datasets as theirs.
The unit energy/latency parameters are obtained from either real-device measurements or synthesized RTL implementation: we measure edge devices' unit energy and latency   repetitively and adopt the mean values; For the ASIC accelerators, the unit parameters are obtained either from ~\cite{eyeriss} or  gate-level simulations using synthesized RTL implementation based on the same CMOS technology.

\begin{scriptsize}
\begin{table}[h!]
\vspace{-0.9em}
\caption{Cross-platform/model/design/dataset settings.}
\vspace{-1em}
\def\arraystretch{1.2}
\centering
% \scriptsize
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Arch/Device}} & {\textbf{}} & \multirow{2}{*}{\textbf{DNNs}$^b$} & {\textbf{Unit}}& {\textbf{Precision}} & {\textbf{Freq.$^e$}}\\
 & {\textbf{Metrics$^a$}} & ~ & {\textbf{Param.$^c$}}& {\textbf{$<$W,A$>$}$^d$} & {\textbf{(MHz)}}\\
\hline
{\textbf{Ultra96}~\cite{ultra96}} & {\textit{E, L, R}} & {Compact} & {Measured}& {$<$11,9$>$} & {220}\\
\hline
{\textbf{Edge TPU}~\cite{edgetpu}} & {\textit{E, L}} & {Compact} & {Measured} & {$<$8,8$>$} & {500}\\
\hline
{\textbf{Jetson TX2}~\cite{edgegpu}} & {\textit{E, L}} & {Compact} & {Measured} & {$<$32,32$>$} & {1300}\\
%\hline
%{\textbf{Pixel 2 XL}} & {-} & {-} & {Compa.} & {-} &{<8,8>}& {2350MHz}\\
\hline
{\textbf{Eyeriss}~\cite{eyeriss}} & {\textit{E, L, R}} & {AlexNet}  & {Reported} & {$<$16,16$>$} & {250}\\
\hline
{\textbf{ShiDianNao}~\cite{du2015shidiannao}} & {\textit{E}} & {Small} & {Synthesized} & {$<$16,16$>$}& {1000}\\
\hline
\end{tabular}
\\
\begin{tablenotes}
\item{$^a$ Metrics -- \textit{E}: energy, \textit{L}: latency, \textit{R}: resource.}
% \item{$^b$ Validation methodology -- Sim: simulated by our Chip predictor, Meas: measured by the device, Rep: reported by the paper }
\item{$b$ DNN benchmarks -- Compact: SK and MB models; AlexNet~\cite{NIPS2012_4824}; and Small: DNNs used in ~\cite{du2015shidiannao} ($<$ five convolutional/fully-connected layers).}
\item{$c$ Methods to obtain the unit parameters.}
\item{$d$ Bit precision for different types of data, i.e., $<$weight, activation$>$}
\item{$e$ Clock frequency for the computation core.}
% \todob{Yang & Cong: check the description}
\end{tablenotes}
\vspace{-0pt}

\label{tab:val_setting}
%\vspace{-0pt}
\vspace{-2em}
\end{table}
\end{scriptsize}

\textbf{Validation of the Predicted Energy and Latency.} \underline{On} \underline{edge devices:} 
%We compare the \textit{DNN-Chip Predictor}'s predicted energy and latency with the measured ones from edge devices under the same settings (see Table~\ref{tab:val_setting}).
Fig.~\ref{fig:val_energy_latency} summarizes the validation results comparing the \textit{DNN-Chip Predictor}'s predicted \textbf{energy} and \textbf{latency} with the measured ones on edge devices and shows that the maximum energy and latency prediction error of our \textit{DNN-Chip Predictor} is 9.17\% and 9.75\% respectively, across the 3 edge devices and 15 DNN models. 
% Note that the energy and latency of the SK1-SK5 are relatively large, because these five models use short-cut paths and reorganization structures~\cite{zhang2019skynet} which are not supported by the edge TPU and thus are processed by the TPU's embedded CPU that is less optimized for DNN operations as compared to the TPU design. 
\underline{On ASIC DNN accelerators:} 
% Fig.~\ref{fig:val_energy_eyeriss} and Table~\ref{tab:val_energy_shidiannao} summarize the validation of our \textit{DNN-Chip Predictor}'s predicted \textbf{energy} over two state-of-the-art ASIC DNN accelerators: Eyeriss~\cite{eyeriss} and ShiDianNao \cite{du2015shidiannao}, respectively, under the same settings. 
For Eyeriss~\cite{eyeriss}, the predicted \textbf{energy} breakdown of AlexNet's convolutional layers is shown in Fig.~\ref{fig:val_energy_eyeriss} (a) with a prediction error $\le 5.15\%$; the DRAM and SRAM accesses prediction error is under $9.64\%$  as shown in Fig.~\ref{fig:val_energy_eyeriss} (b).
%the number of DRAM/SRAM accesses are show in Fig.~\ref{fig:val_energy_eyeriss} (b), and
%we first compare the predicted energy breakdown of AlexNet's convolutional layers, showing that the maximum difference is $5.15\%$ and $1.64\%$, shown in Fig.~\ref{fig:val_energy_eyeriss} (a). Then we further compare the number of DRAM/SRAM accesses as shown in Fig.~\ref{fig:val_energy_eyeriss} (b), and observe the DRAM and SRAM accesses difference is under $9.56\%$ and $9.54\%$ respectively.
% The relatively larger error of the first convolutional layer is caused by the employed larger stride of 4. Specifically, a larger stride leads to a less utilization of the inputs fetched from the SRAM, and our predictor considers only the commonly used strides of 1 and 2, which are more often seen in recent DNN models, for simplicity. Note our \textit{Predictor} can be straightforwardly extended to cover cases of using other stride values. 
The \textbf{energy} validation results over ShiDianNao~\cite{du2015shidiannao} are listed in Table~\ref{tab:val_energy_shidiannao}. The energy breakdown of the four IPs, averaging over 10 DNN shows that the prediction error is under 9.59\%. 
% Note that the prediction error is mainly due to the fact that there can be some slight difference between our adopted commercial CMOS IP library with that in ~\cite{du2015shidiannao} although both use the same technology. 
Table~\ref{tab:val_eyeriss_lat} compares the \textbf{latency} of executing AlexNet's convolutional layers on Eyeriss~\cite{eyeriss}, showing that the largest prediction error in latency is $4.12\%$. The predicted latency is smaller than the paper-reported ones, because accessing the memory multiple times for one single data wordline is not considered in \textit{DNN-Chip Predictor}, which can be included by recording the corresponding memory data arrangements.


\begin{figure}[h]
\vspace{-1em}
    \centerline{\includegraphics[width=0.9\linewidth]{fig/val_lat_2.pdf}}
    \vspace{-1em}
    \caption{The energy \& latency prediction error of the 15 DNNs with various capacities on the 3 edge devices.}
    \label{fig:val_energy_latency}
    \vspace{-1em}
\end{figure}

\begin{figure}[h]
\vspace{-1em}
    \centerline{\includegraphics[width=0.9\linewidth]{fig/eyeriss_all.pdf}}
    \vspace{-1.2em}
    \caption{The prediction error over Eyeriss: (a) The energy breakdown for the first and fifth convolution layers and (b) the \# of DRAM and SRAM accesses.}
    \label{fig:val_energy_eyeriss}
    \vspace{-1.2em}
\end{figure}

\begin{table}[h!]
\vspace{-1em}
\caption{The energy prediction error over ShiDianNao.}
\def\arraystretch{1.2}
\centering
\tiny
\vspace{-1.9em}
\begin{tabular}{|c|c|c|c|c|}
\hline
{\textbf{IP}} & {\textbf{Computation}} & {\textbf{Input SRAM}} & {\textbf{Output SRAM}} & {\textbf{Weight SRAM}}  \\
\hline
\multirow{1}{*}{Predicted (\%)} & {89.2} & {7.4} & {1.7} & {1.6}\\
\hline
\multirow{1}{*}{Paper-reported (\%)} & {89.0} & {8.0} & {1.6} & {1.5} \\
\hline
\multirow{1}{*}{\textbf{Prediction error}} & {0.35\%} & {-7.19\%} & \textbf{{9.59\%}} & {7.87\%} \\
\hline
\end{tabular}
%\vspace{-0pt}
%\vspace{-0pt}
\vspace{-2em}
\label{tab:val_energy_shidiannao}
\end{table}


\begin{table}[h!]
\vspace{-0.5em}
\caption{The latency prediction error over Eyeriss.}
\vspace{-1em}
\def\arraystretch{1.2}
\centering
%\fontsize{7.5}{9}\selectfont
% \scriptsize
\tiny
\begin{tabular}{|c|c|c|c|c|c|}
\hline
{\textbf{AlexNet Layer}} & {\textbf{CONV1}} & {\textbf{CONV2}} & {\textbf{CONV3}} & {\textbf{CONV4}} & {\textbf{CONV5}} \\
\hline
\multirow{1}{*}{Predicted latency (ms)} & {16.04} & {37.58} & {21.09} & {15.59} & {9.79}\\
\hline
\multirow{1}{*}{Paper-reported latency (ms)} & {16.5} & {39.2} & {21.8} & {16} & {10}\\
\hline
\multirow{1}{*}{\textbf{Prediction error}} & \textit{{-2.88\%}} & {\textbf{-4.12\%}} & \textit{{-3.24\%}} & \textit{{-2.56\%}} & \textit{{-2.14\%}}\\
\hline
\end{tabular}
\vspace{-2em}
\label{tab:val_eyeriss_lat}
\end{table}


\vspace{-1.5em}
\textbf{Validation of the Predicted Resource Consumption.} 
Table~\ref{tab:val_resource} shows the predicted resource consumption of \ul{Ultra96 FPGA}. Specifically, the predicted resource consumption for the two critical on-chip resources of FPGAs, DSP48E and BRAM18K, is validated against those obtained from the post-implementation utilization reports, and have a prediction error of smaller than $4.2\%$ and $3.2\%$ for the DSP48E and BRAM18K, respectively. 
% Note that the DSP48Es are the embedded multipliers in the FPGA and the BRAM18K is the main on-chip memory resource in the FPGA. In addition, the 6 cases, i.e., Bg. 1-6, in Table~\ref{tab:val_resource} correspond to 6 designs under varied resource budgets. 
For the validation over ASIC DNN accelerators, we evaluate the MAC utilization. Estimated MAC utilization among the five convolutional layers of AlexNet is the same as the paper-reported ones for \ul{Eyeriss}~\cite{eyeriss}. Since the MAC utilization is only determined by the parallelism level of the PE array in Eyeriss's case.






\begin{table}[h!]
\vspace{-1em}
\caption{
% Resource Model validation for DSP48E and BRAM18K on Ultra96
The resource consumption prediction error over Ultra96 FPGA board.}
\vspace{-1em}
\def\arraystretch{1.2}
\centering
%\fontsize{7.5}{9}\selectfont
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
{\textbf{Resource type}}& {Val.}  & {\textbf{Bg. 1}} & {\textbf{Bg. 2}} & {\textbf{Bg. 3}} & {\textbf{Bg. 4}} & {\textbf{Bd. 5}} & {\textbf{Bd. 6}} \\
\hline
\multirow{3}{*}{DSP48E} & Predicted & 35 & 69 & 141 & 213 & 285 & 331 \\
 & Measured & 36 & 72 & 144 & 216 & 288 & 360 \\
 & \textbf{Error} & \-3.2\% & \textbf{-4.2\%} & -2.4\% & -1.2\% & -1.0\% & \-0.8\% \\
\hline
\multirow{3}{*}{DRAM18K} & Predicted & 65 & 87 & 175 & 265 & 354 & 446\\
 & Measured & 64 & 86 & 173 & 259 & 346 & 432 \\
 & \textbf{Error} & +1.0\% & +0.8\% & +1.2\% & +2.2\% & +2.4\% & \textbf{+3.2\%} \\
\hline
\end{tabular}
%\vspace{-0pt}
%\vspace{-0pt}
\vspace{-1.7em}
\label{tab:val_resource}
\end{table}


% \textbf{Validation of the Predicted Resource Consumption.} 
% Table~\ref{tab:val_resource} shows the predicted resource consumption of \ul{Ultra96 FPGA}. Specifically, the predicted resource consumption for the two critical on-chip resources of FPGAs, DSP48E and BRAM18K, is validated against those obtained from the post-implementation utilization reports, and have a prediction error of smaller than $4.2\%$ and $3.2\%$ for the DSP48E and BRAM18K, respectively. 
% % Note that the DSP48Es are the embedded multipliers in the FPGA and the BRAM18K is the main on-chip memory resource in the FPGA. In addition, the 6 cases, i.e., Bg. 1-6, in Table~\ref{tab:val_resource} correspond to 6 designs under varied resource budgets. 
% For the validation over ASIC DNN accelerators, we evaluate the MAC utilization. Estimated MAC utilization among the five convolutional layers of AlexNet is the same as the paper-reported ones for \ul{Eyeriss}~\cite{eyeriss}. Since the MAC utilization is only determined by the parallelism level of the PE array in Eyeriss's case.


\textbf{A Case Study of Using the \textit{DNN-Chip Predictor}.} 
We further employ the \textit{DNN-Chip Predictor} to design an FPGA based DNN accelerator using a naive exhaustive search method for evaluating its efficiency and effectiveness. We first use the coarse-grained \textit{DNN-Chip Predictor} to simulate 4.6 million design choices of different architectures and dataflows, which takes only 0.8 hour thanks to the coarse-grained prediction's analytical nature. For each remaining candidate from the previous step, we spend 0.57 hour to estimate the fine-grained performance. The optimal candidates after these two steps are passed to Vivado for an implementation on a state-of-the-art FPGA board Ultra96 ~\cite{ultra96}. Real-measured results demonstrate that the resulting accelerator achieves 41.82\% throughput improvement and 2.4$\times$ idle cycles reduction than an award wining state-of-the-art FPGA based DNN accelerator ~\cite{zhang2019skynet} given the same DNN models and FPGA board.

% \todob{
% \subsubsection{Different architectures on ASIC}
% \begin{itemize}
%     \item Against Eyeriss (paper reported)
%     For the validation against Eyeriss architecture~\cite{eyeriss}, we use AlexNet

%     \item Against Shidiannao (synthesized)
%     \item Against SmartExchange (synthesized)
%     \item Against TPU (edge-TPU-measured and synthesized)
% \end{itemize}
% \subsubsection{Against FPGA (measured)}
% \subsubsection{Against mobile device, due Aug 20}
% \begin{itemize}
%     \item Luke: deploy the inference on mobile for: (1) 6~10 NN models with 2 backbone (mobileNet and another one) (2) separated conv layers.
%     \item  Yue: power and latency measurement for (1) and (2)
% \end{itemize}

% \subsubsection{Against GPU (edge-GPU-measured)}
% }

% \begin{figure}[h]
%     \centerline{\includegraphics[width=50mm]{fig/val_shidiannao.png}}
%     \vspace{-1em}
%     \caption{\textbf{Energy Validation results for the architecture on Shidiannao.~\cite{du2015shidiannao}} \todob{By Yang}}
%     \vspace{-1.1em}
%     \label{fig:val_shidiannao}
% \end{figure}

% \textbf{Validation on FPGA board} We compare our models' predicted latency with FPGA measured ones under the same DNN model and hardware configurations~\cite{zhang2019skynet}. Specifically, for the FPGA one we use the open source implementation of the award winner~\cite{zhang2019skynet} in a state-of-the-art design contest~\cite{dac-contest}.\\


% \begin{figure}[h]
%     \centerline{\includegraphics[width=80mm]{fig/val_resource.pdf}}
%     \vspace{-1em}
%     \caption{\textbf{Resource Model validation for DSP48E and BRAM18K on Ultra96}}
%     \vspace{-1.1em}
%     \label{fig:val_resource}
% \end{figure}



% \textbf{Validation of the Predicted Latency.} \textbf{On edge platforms:} The latency prediction of the \textit{DNN-Chip Predictor} is validated over the measured results of the 15 DNN models on 3 edge devices as summarized in Fig.~\ref{fig:val_lat}. We can see that
% \textbf{the maximum latency prediction error of our \textit{DNN-Chip Predictor} is $\boldsymbol{9.75\%}$ over the 3 platforms and 15 DNN models}. Specifically, the prediction errors are from $0.89\%$ to $9.75\%$, $1.78\%$ to $5.98\%$, and $2.92\%$ to $9.44\%$, when using the edge GPU, the Ultra96 FPGA board, and the edge TPU, respectively, and the corresponding average prediction error is $4.85\%$, $3.73\%$, and $6.57\%$, respectively. Similar to the case in the validation of energy prediction, the latency of the SkyNet and SK1-SK4 models are relatively large, because these five models use structures (i.e., short-cut and reorganization)~\cite{zhang2019skynet} which are not supported by the edge TPU and thus are processed by the TPU's embedded CPU that is not optimized for DNN operations as compared to the TPU design. 

% we do not consider the real data arrangement in memory. In some corner cases, the accelerator needs to access the memory multiple times for one wordline of data because the data is physically stored in multiple wordlines in memory.  
% This could be solved by recording the memory data arrangement in our proposed chip predictor, . Trading-off between the predictor's time efficiency and prediction accuracy, we use a simple memory model in current design. 

==> tex/_4-Experiment.tex <==
\section{Experiment Results}
\label{sec:exp}
% In this section, we validate the prediction accuracy and effectiveness for the proposed \textit{Chip Predictor} by (1) comparing its predicted performance with real-device measured or reported one of state-of-the-art accelerators in terms of energy consumption, latency, and resource consumption; (2) showing the performance of the optimized DNN accelerator design with design space exploration driven by \textit{Chip Predictor}.
In this section, we validate the proposed \textit{Chip Predictor} by comparing its predicted performance with real-device measured and the state-of-the-art accelerators in terms of energy consumption, latency, and resource consumption. 

Specifically, extensive experiments on 3 edge devices and 15 DNN models show that the \textit{Chip Predictor}'s prediction error for energy, latency, and resource consumption is less than $10\%$ under various design settings and datasets.
\subsection{Experiment Setup.}
Table~\ref{tab:val_setting} summarizes the \textit{Chip Predictor}'s experiment setting, including the platforms/accelerators, performance metrics, DNN models, methods to obtain the unit parameters, employed precision for the weights and activations, and frequency of the corresponding computation core. \textbf{Methodology:} In order to conduct a solid validation, we validate the \textit{Chip Predictor} by comparing its predicted performance with actual device-measured ones on \ul{3 edge devices} (Ultra96 FPGA~\cite{ultra96}, edge TPU~\cite{edgetpu}, Jetson TX2~\cite{edgegpu}) and paper-reported ones of \ul{2 published ASIC DNN accelerators} (Eyeriss~\cite{eyeriss} and ShiDianNao~\cite{du2015shidiannao}), when adopting the same experiment settings (e.g., clock frequency, DNN model and dataset, bit precision, architecture design, and dataflow, etc). \textbf{Benchmark DNN models and datasets:} For the 3 edge devices, we consider 15 representative compact/light-weight DNN models (see Table~\ref{tab:dnn_sk} and Table~\ref{tab:dnn_mb}, where the models in Table~\ref{tab:dnn_mb} use the ImageNet dataset~\cite{Deng09imagenet} and the models in Table~\ref{tab:dnn_sk} use the dataset in the System Design Contest of the DAC 2019 conference ~\cite{dac-contest}); For the 2 published DNN accelerators, we use the same benchmark models and datasets as the original papers.
\textbf{Unit parameters:} The unit energy/latency parameters are obtained through either real-device measurement or synthesized RTL implementation as mentioned in Section~\ref{sec:chip_pred}. Specifically, for the 3 edge devices, we measure the unit energy and latency when running the basic IP operations (such as the memory accesses and the MAC computation) repetitively and adopt the mean values as unit parameters. Specifically, we run the basic IP operations over 128 sets of experiments. For memory accesses, we change the clock frequency, memory volume, port width, bit precision, and burst read length; for the MAC operations, the clock frequency, total number of MACs and the parallelism of MACs are changed.
 For the ASIC DNN accelerators, the unit parameters are obtained either form the paper~\cite{eyeriss} or from gate-level simulations of the synthesized RTL implementation based on the same CMOS technology.

\begin{scriptsize}
\begin{table}[h!]
\caption{Experiment settings for the \textit{Chip Predictor}'s cross-platform/model/design/dataset validation.}
\vspace{-1em}
\def\arraystretch{1.2}
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Arch/Device}} & {\textbf{}} & \multirow{2}{*}{\textbf{DNNs}$^b$} & {\textbf{Unit}}& {\textbf{Precision}} & {\textbf{Freq.$^e$}}\\
 & {\textbf{Metrics$^a$}} & ~ & {\textbf{Param.$^c$}}& {\textbf{<W,A>}$^d$} & {\textbf{(MHz)}}\\
\hline
{\textbf{Ultra96}~\cite{ultra96}} & {\textit{E, L, R}} & {Compact} & {Measured}& {<11, 9>} & {220}\\
\hline
{\textbf{Edge TPU}~\cite{edgetpu}} & {\textit{E, L}} & {Compact} & {Measured} & {<8, 8>} & {500}\\
\hline
{\textbf{Jetson TX2}~\cite{edgegpu}} & {\textit{E, L}} & {Compact} & {Measured} & {<32, 32>} & {1300}\\
%\hline
%{\textbf{Pixel 2 XL}} & {-} & {-} & {Compa.} & {-} &{<8,8>}& {2350MHz}\\
\hline
{\textbf{Eyeriss}~\cite{eyeriss}} & {\textit{E, L, R}} & {AlexNet}  & {Reported} & {<16, 16>} & {250}\\
\hline
{\textbf{ShiDianNao}~\cite{du2015shidiannao}} & {\textit{E}} & {Small} & {Synthesized} & {<16, 16>}& {1000}\\
\hline
\end{tabular}
\\
\begin{tablenotes}
\item{$^a$ Metrics -- \textit{E}: energy, \textit{L}: latency, \textit{R}: resource.}
% \item{$^b$ Validation methodology -- Sim: simulated by our Chip predictor, Meas: measured by the device, Rep: reported by the paper }
\item{$b$ DNN benchmarks -- Compact: See the 15 compact DNN models in Table~\ref{tab:dnn_sk} and Table~\ref{tab:dnn_mb}; AlexNet~\cite{NIPS2012_4824}; and Small: DNNs used in ~\cite{du2015shidiannao} (< five convolutional/fully-connected layers).}
\item{$c$ Methods to obtain the unit parameters.}
\item{$d$ Bit precision for different types of data, i.e., <weight precision, activation precision>}
\item{$e$ Clock frequency for the computation core.}
% \todob{Yang & Cong: check the description}
\end{tablenotes}
\vspace{-0pt}

\label{tab:val_setting}
%\vspace{-0pt}
%\vspace{-2.7em}
\end{table}
\end{scriptsize} 
\subsection{Validate \textit{Chip Predictor}'s Prediction Accuracy.}



\subsection{Validate \textit{Chip Predictor}'s Effectiveness to Drive Design Space Exploration}





\textbf{Validation of the Predicted Energy Consumption.} 
\textbf{On edge platforms:} We compare the \textit{Chip Predictor}'s predicted energy with the measured ones from three edge devices (including Ultra96 FPGA~\cite{ultra96}, edge TPU~\cite{edgetpu}, and Jetson TX2 (edge GPU)~\cite{edgegpu}) under the same settings (see Table~\ref{tab:val_setting}). Fig. ~\ref{fig:val_energy} summarizes the validation results, and shows that \textbf{the maximum prediction error of our \textit{Chip Predictor} is $\boldsymbol{9.17\%}$ on the 3 platforms and 15 DNN models}. Specifically, the prediction error ranges from $0.89\%$ to $8.13\%$, $2.12\%$ to $7.67\%$, and $2.72\%$ to $9.17\%$, for the cases using the edge GPU, the Ultra96 FPGA board, and the edge TPU, respectively, and the corresponding average prediction error is $5.40\%$, $5.20\%$, and $6.05\%$, respectively. Note that the energy consumption of the SkyNet and SK1-SK4 models are relatively large, because these five models use short-cut paths and reorganization structures~\cite{zhang2019skynet} which are not supported by the edge TPU and thus are processed by the TPU's embedded CPU that is less optimized for DNN operations as compared to the TPU design. 




% The resulting difference for \ul{Ultra96 FPGA}~\cite{ultra96} is less than $\leq7.67\%$. Our predicted energy differs from the \ul{edge TPU}~\cite{edgetpu}-measured ones by $\leq9.17\%$. SkyNet to SK4 models use short-cut path and reorganization~\cite{zhang2019skynet} which are not supported by edge TPU and are processed by embedded CPU in the TPU device. Therefore, the energy of these five models consume larger energy than other models. 
% For \ul{Jetson TX2}~\cite{edgegpu}, the prediction error is within $\leq8.13\%$ as shown in Fig.~\ref{fig:val_energy}. 
% %, and the prediction error is relatively larger because the CPU control is not accurately modeled in our Chip predictor. 
% The \ul{average energy prediction error} is $5.20\%$, $6.05\%$, and $5.40\%$ for the Ultra96 FPGA~\cite{ultra96}, edge TPU~\cite{edgetpu}, and Jetson TX2~\cite{edgegpu} respectively. The relatively larger prediction error for edge TPU and Jetson TX2 than Ultra96 FPGA is because our model does not have CPU control run-time simulation for these "wrapped" commercial devices while CPU control counts for a larger percent of energy for edge TPU and Jetson TX2 than FPGA. 
% To be more specific, edge TPU~\cite{edgetpu} and Jetson TX2~\cite{edgegpu} offload the control of on-chip computation and data loading/unloading to embedded CPU (because user-defined layers with operation are not supported by edge TPU and GPU) while Ultra96 FPGA does not. 
%CPU control counts for a relatively larger percent (in the total data loading/unloading control) for edge TPU and Jetson TX2 than FPGA because for FPGA, the on-chip computation and BRAM memory access is not controlled by CPU, but for Edge TPU and GPU, on-chip computation/control workload (e.g. user-defined layers with operations not supported by edge TPU) is offloaded onto the embedded CPU core to operate.
\textbf{Over ASIC DNN accelerators:} 
Fig.~\ref{fig:val_energy_eyeriss} and Table~\ref{tab:val_energy_shidiannao} summarize the validation of our \textit{Chip Predictor}'s predicted energy over two state-of-the-art ASIC DNN accelerators: Eyeriss~\cite{eyeriss} and ShiDianNao \cite{du2015shidiannao}, respectively, under the same settings. \ul{For Eyeriss}~\cite{eyeriss}, we first compare the predicted energy breakdown of AlexNet's first and fifth convolutional layers, showing that the maximum difference is $5.15\%$ and $1.64\%$, respectively as shown in Fig.~\ref{fig:val_energy_eyeriss} (a). Because memory accesses dominate the energy consumption~\cite{eyeriss}, we further compare the number of DRAM/SRAM accesses as shown in Fig.~\ref{fig:val_energy_eyeriss} (b), and show that the difference between the predicted number of DRAM accesses and Eyeriss's measured results is between $2.18\%$ and $9.56\%$ , while the difference in terms of SRAM accesses is less than $9.54\%$. The relatively larger error of the first convolutional layer is caused by the employed larger stride of 4. Specifically, a larger stride leads to a less utilization of the inputs fetched from the SRAM, and our predictor considers only the commonly used strides of 1 and 2, which are more often seen in recent DNN models, for simplicity. Note our \textit{Predictor} can be straightforwardly extended to cover cases of using other stride values. The validation results over \ul{ShiDianNao}~\cite{du2015shidiannao} are listed in Table~\ref{tab:val_energy_shidiannao}. The energy breakdown of the four IPs, which is averaged over 10 DNN benchmarks as in~\cite{du2015shidiannao}, shows that the prediction error is no large than 9.59\%. Note that the prediction error is mainly due to the fact that there can be some slight difference between our adopted commercial CMOS IP library with that in ~\cite{du2015shidiannao} although both use the same technology. 

% Although we choose the same technology to get the unit parameter for the \textit{Chip Predictor}, there still exists a difference between our CMOS library and that in the original design which brings the difference. 


\begin{figure}[h]
\vspace{-1.4em}
    \centerline{\includegraphics[width=1.15\linewidth]{fig/val_energy.pdf}}
    \vspace{-1em}
    \caption{\textbf{The energy prediction error of the \textit{Chip Predictor} when using the 15 DNN models in Table~\ref{tab:dnn_sk} and Table~\ref{tab:dnn_mb} running on 3 edge devices (Ultra 96 FPGA board~\cite{ultra96}, Edge TPU~\cite{edgetpu}, and Edge GPU (Jetson TX2)~\cite{edgegpu}.}}
%\todob{add precision, adjust color, height/weight ratio, fig size, font size, legend size, add text for the largest/smallest prediction error} 
    \vspace{-1.6em}
    \label{fig:val_energy}
\end{figure}

\begin{figure}[!t]
\vspace{-1.9em}
\captionsetup[subfigure]{labelformat=empty}
%    \vspace{-1em}
    \centering
    \subfloat{\includegraphics[width=62mm]{fig/eyeriss_energy.pdf} }\hspace{-10pt}
    \begin{center}
    (a) \\
    \end{center}
    \subfloat{\includegraphics[width=62mm]{fig/eyeriss_sram_dram.pdf}}
    \begin{center}
    (b) \\
    \end{center}
    \vspace{-1em}
    \caption{\textbf{
    The energy prediction error of the \textit{Chip Predictor} when using the architecture of the state-of-the-art DNN accelerator, Eyeriss~\cite{chen2017eyeriss}: The energy breakdown for the first and fifth convolutional layers (a) and the $\#$ of DRAM and SRAM accesses (b) }}
    \vspace{-1em}
    \label{fig:val_energy_eyeriss}
\end{figure}


% \begin{figure}[!t]
% \vspace{-1.2em}
% \captionsetup[subfigure]{labelformat=empty}
%     %\vspace{-1em}
%     \centering
%     \subfloat{{\includegraphics[width=20mm]{fig/shidiannao_energy.pdf} }}\hspace{5pt}
%     \subfloat{{\includegraphics[width=20mm]{fig/shidiannao_dram_sram.pdf} }}
%     \vspace{-1em}
%     \caption{\textbf{Validation of the \textit{Chip Predictor}'s energy prediction performance over ShiDianNao~\cite{du2015shidiannao}: The energy breakdown over 10 benchmarks (left) and energy of 10 benchmarks (right) of  }}
%     \vspace{-1.5em}
%     \label{fig:val_energy_shidiannao}
% \end{figure}


\begin{table}[h!]
\vspace{-1em}
\caption{\textbf{The energy prediction error of the \textit{Chip Predictor} when using the architecture of the state-of-the-art DNN accelerator, ShiDianNao~\cite{du2015shidiannao}: The energy breakdown over 10 benchmarks.}}
\def\arraystretch{1.2}
\centering
%\fontsize{7.5}{9}\selectfont
\scriptsize
\begin{tabular}{|c|c|c|c|c|}
\hline
{\textbf{IP}} & {\textbf{Computation}} & {\textbf{Input SRAM}} & {\textbf{Output SRAM}} & {\textbf{Weight SRAM}}  \\
\hline
\multirow{1}{*}{Predicted (\%)} & {89.2} & {7.4} & {1.7} & {1.6}\\
\hline
\multirow{1}{*}{Paper-reported (\%)} & {89.0} & {8.0} & {1.6} & {1.5} \\
\hline
% \multirow{1}{*}{Prediction error} & {0.35\%} & {-7.19\%} & \textbf{{9.59\%}} & {7.87\%} \\
\multirow{1}{*}{\textbf{Prediction error}} & {\textbf{0.35\%}} & {\textbf{-7.19\%}} & \textbf{{9.59\%}} & {\textbf{7.87\%}} \\
\hline
\end{tabular}
%\vspace{-0pt}
%\vspace{-0pt}
\vspace{-1.7em}
\label{tab:val_energy_shidiannao}
\end{table}


% \begin{table}%[!b]
% \centering
% \vspace{3mm}
% \small
% \setlength\tabcolsep{2pt}
% \begin{tabular}{@{}c | cc c cc c cc c cc@{}}\toprule
% \multirow{2}{*}{Layer}& \multicolumn{2}{c}{comp.} & \phantom{x}& \multicolumn{2}{c}{RF} & \phantom{x}& \multicolumn{2}{c}{NoC} & \phantom{x}& \multicolumn{2}{c}{GB}\\ 
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
% & Meas. & Pred. && Meas. & Pred. && Meas. & Pred. && Meas. & Pred.  \\ 
% \midrule
% \multirow{1}{*}{CONV1}
% $ $ & 16.7\% & 18.7\% && 79.6\% & 74.4\% && 1.7\% & 4.8\% && 2.0\% & 2.0\%\\
% % \midrule
% \multirow{1}{*}{\textbf{$\Delta$}}
% $ $ & \multicolumn{2}{c}{\textbf{2.08\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-5.15\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{3.10\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-0.03\%}}\\
% \midrule
% \multirow{1}{*}{CONV5}
% $ $ & 7.3\% & 7.5\% && 80.3\% & 79.1\% && 5.3\% & 7.0\% && 7.0\% & 6.3\%\\
% % \midrule
% \multirow{1}{*}{\textbf{$\Delta$}}
% $ $ & \multicolumn{2}{c}{\textbf{0.26\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-1.16\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{1.64\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-0.74\%}}\\
% \bottomrule
% \end{tabular}
% \caption{\textbf{The energy breakdown from Eyeriss~\cite{chen2017eyeriss} and our models, for the CONV1 and CONV5 of AlexNet\cite{NIPS2012_4824}.}}
% \label{table:val_eyeriss_energy}
% \vspace{-2.2em}
% \end{table}
% Validation of the Predicted Energy Consumption.

\textbf{Validation of the Predicted Latency.} \textbf{On edge platforms:} The latency prediction of the \textit{Chip Predictor} is validated over the measured results of the 15 DNN models on 3 edge devices as summarized in Fig.~\ref{fig:val_lat}. We can see that
\textbf{the maximum latency prediction error of our \textit{Chip Predictor} is $\boldsymbol{9.75\%}$ over the 3 platforms and 15 DNN models}. Specifically, the prediction errors are from $0.89\%$ to $9.75\%$, $1.78\%$ to $5.98\%$, and $2.92\%$ to $9.44\%$, when using the edge GPU, the Ultra96 FPGA board, and the edge TPU, respectively, and the corresponding average prediction error is $4.85\%$, $3.73\%$, and $6.57\%$, respectively. Similar to the case in the validation of energy prediction, the latency of the SkyNet and SK1-SK4 models are relatively large, because these five models use structures (i.e., short-cut and reorganization)~\cite{zhang2019skynet} which are not supported by the edge TPU and thus are processed by the TPU's embedded CPU that is not optimized for DNN operations as compared to the TPU design. 

% The predicted latency and \ul{FPGA}~\cite{ultra96} measured ones differ from $1.78\%$ to $5.98\%$. \ul{Edge TPU}~\cite{edgetpu} latency prediction has an error of $\leq 9.44\%$. \ul{Jetson TX2's}~\cite{edgegpu} prediction error is $0.89\%$ to $9.75\%$ different from the measured ones. 
% The \ul{average latency prediction error} is $3.73\%$, $6.57\%$, and $4.85\%$ for the Ultra96 FPGA~\cite{ultra96}, edge TPU~\cite{edgetpu}, and Jetson TX2~\cite{edgegpu} respectively. 
% The relatively larger prediction error for TPU and GPU than FPGA is also because of the lack of CPU control estimation which counts for a larger percent of latency for TPU and GPU than FPGA. 
%The relatively larger prediction error for TPU and GPU than FPGA is because our model does not have CPU control run-time simulation for these "wrapped" commercial devices. CPU control counts for a relatively larger percent (in the total data loading/unloading control) for edge TPU and Jetson TX2 than FPGA because for FPGA, the on-chip computation and BRAM memory access is not controlled by CPU, but for Edge TPU and GPU, on-chip computation/control workload (e.g. user-defined layers with operations not supported by edge TPU) is offloaded onto the embedded CPU core to operate.
\textbf{Over ASIC DNN accelerators:} 
Table~\ref{tab:val_eyeriss_lat} compares the latency of executing AlexNet's five convolutional layers on \ul{Eyeriss}~\cite{eyeriss}, showing that the largest prediction error in latency is $4.12\%$. The predicted latency by our \textit{Chip Predictor} is smaller than the paper-reported measurements, because our \textit{Chip Predictor} does not consider the special scenarios when the accelerator needs to access the memory multiple times for one single wordline of data. Such scenarios are only needed to consider when one wordline of data is physically stored in multiple wordlines of the memory. While our \Textit{Chip Predictor} can be extended to include such cases by recording the corresponding memory data arrangements, the current version do not consider such corner cases for better trading-off the predictor's time efficiency and prediction accuracy.

% we do not consider the real data arrangement in memory. In some corner cases, the accelerator needs to access the memory multiple times for one wordline of data because the data is physically stored in multiple wordlines in memory.  
% This could be solved by recording the memory data arrangement in our proposed chip predictor, . Trading-off between the predictor's time efficiency and prediction accuracy, we use a simple memory model in current design. 


\begin{figure}[h]
\vspace{-1.3em}
    \centerline{\includegraphics[width=1.15\linewidth]{fig/val_lat_2.pdf}}
    \vspace{-1em}
    \caption{\textbf{The latency prediction error of the \textit{Chip Predictor} when using 15 DNN models on 3 edge devices including Ultra 96 FPGA board, Edge TPU, and Jetson TX2 (edge GPU).}}
%\todob{add precision, adjust color, height/weight ratio, fig size, font size, legend size, add text for the largest/smallest prediction error} 
    \vspace{-1.1em}
    \label{fig:val_lat}
\end{figure}

% \begin{figure}[h]
%     \centerline{\includegraphics[width=75mm]{fig/val_eyeriss_latency.pdf}}
%     \vspace{-1em}
%     \caption{\todob{Yue: change it to table}\textbf{Validation results for processing latency of CONV1 to CONV5 in AlexNet against Eyeriss.~\cite{eyeriss}}}
%     \vspace{-1.1em}
%     \label{tab:val_eyeriss_lat}
% \end{figure}

\begin{table}[h!]
% \vspace{-0.2em}
\caption{\textbf{The latency prediction error of the \textit{Chip Predictor} when using the architecture of Eyeriss~\cite{eyeriss}: latency when processing the five convolutional layers of AlexNet}.}
\vspace{-0.6em}
\def\arraystretch{1.2}
\centering
%\fontsize{7.5}{9}\selectfont
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
{\textbf{AlexNet Layer}} & {\textbf{CONV1}} & {\textbf{CONV2}} & {\textbf{CONV3}} & {\textbf{CONV4}} & {\textbf{CONV5}} \\
\hline
\multirow{1}{*}{Predicted latency (ms)} & {16.04} & {37.58} & {21.09} & {15.59} & {9.79}\\
\hline
\multirow{1}{*}{Paper-reported latency (ms)} & {16.5} & {39.2} & {21.8} & {16} & {10}\\
\hline
\multirow{1}{*}{\textit{Prediction error}} & \textit{{-2.88\%}} & {\textbf{-4.12\%}} & \textit{{-3.24\%}} & \textit{{-2.56\%}} & \textit{{-2.14\%}}\\
\hline
\end{tabular}
%\vspace{-0pt}
%\vspace{-0pt}
\vspace{-1.5em}
\label{tab:val_eyeriss_lat}
\end{table}



% \todob{
% \subsubsection{Different architectures on ASIC}
% \begin{itemize}
%     \item Against Eyeriss (paper reported)
%     For the validation against Eyeriss architecture~\cite{eyeriss}, we use AlexNet

%     \item Against Shidiannao (synthesized)
%     \item Against SmartExchange (synthesized)
%     \item Against TPU (edge-TPU-measured and synthesized)
% \end{itemize}
% \subsubsection{Against FPGA (measured)}
% \subsubsection{Against mobile device, due Aug 20}
% \begin{itemize}
%     \item Luke: deploy the inference on mobile for: (1) 6~10 NN models with 2 backbone (mobileNet and another one) (2) separated conv layers.
%     \item  Yue: power and latency measurement for (1) and (2)
% \end{itemize}

% \subsubsection{Against GPU (edge-GPU-measured)}
% }

% \begin{figure}[h]
%     \centerline{\includegraphics[width=50mm]{fig/val_shidiannao.png}}
%     \vspace{-1em}
%     \caption{\textbf{Energy Validation results for the architecture on Shidiannao.~\cite{du2015shidiannao}} \todob{By Yang}}
%     \vspace{-1.1em}
%     \label{fig:val_shidiannao}
% \end{figure}

% \textbf{Validation on FPGA board} We compare our models' predicted latency with FPGA measured ones under the same DNN model and hardware configurations~\cite{zhang2019skynet}. Specifically, for the FPGA one we use the open source implementation of the award winner~\cite{zhang2019skynet} in a state-of-the-art design contest~\cite{dac-contest}.\\

\textbf{Validation of the Predicted Resource Consumption.} 
Table~\ref{tab:val_resource} summarizes the \textit{Chip Predictor}'s predicted resource consumption of \ul{Ultra96 FPGA}~\cite{ultra96}. Specifically, the predicted resource consumption for the two critical on-chip resources of FPGAs, DSP48E and BRAM18K, is validated against those obtained from the post-implementation utilization reports, and have a prediction error of smaller than $4.2\%$ and $3.2\%$ for the DSP48E and BRAM18K, respectively. Note that the DSP48Es are the embedded multipliers in the FPGA and the BRAM18K is the main on-chip memory resource in the FPGA. In addition, the 6 cases, i.e., Bg. 1-6, in Table~\ref{tab:val_resource} correspond to 6 designs under varied resource budgets. 
% For example,  
% The tuning parameters are the resource budget for each of the 6 designs, e.g. design 6 is given the budget of 100% of the DSP and BRAM on Chip, design 5 is only given 50% of the DSP and BRAM on Chip.
% The post-synthesis optimization of Vivado may change part of the buffers' implementation from BRAM to LUTRAM which causes the BRAM prediction error. Although the Chip Predictor precisely estimates the DSP48E resource for computational IPs (nearly 0\% prediction error), the memory address calculation in memory IPs may use larger amount of DSP48E resulting in the DSP48E prediction error. 
%The prediction error of BRAM18K comes from the inaccurate prediction for the post-synthesis optimization of Vivado which changes part of the buffers' implementation from BRAM to LUTRAM; the prediction error of DSP48E comes from the inaccurate prediction for the DSP48E consumption for memory address calculation.   
For the validation over ASIC DNN accelerators, we consider the MAC utilization as the validation metric. Estimated MAC utilization among the five convolutional layers of AlexNet is the same as the paper-reported ones for \ul{Eyeriss}~\cite{eyeriss}. Thie is because the MAC utilization is only determined by the parallelism level of the PE array in Eyeriss's case.

% \begin{figure}[h]
%     \centerline{\includegraphics[width=80mm]{fig/val_resource.pdf}}
%     \vspace{-1em}
%     \caption{\textbf{Resource Model validation for DSP48E and BRAM18K on Ultra96}}
%     \vspace{-1.1em}
%     \label{fig:val_resource}
% \end{figure}

\begin{table}[h!]
\caption{\textbf{
% Resource Model validation for DSP48E and BRAM18K on Ultra96
The resource consumption prediction error of the \textit{Chip Predictor}'s on the Ultra96 FPGA board when considering 6 different designs given 6 different resource budgets.}}
\vspace{-1em}
\def\arraystretch{1.2}
\centering
%\fontsize{7.5}{9}\selectfont
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
{\textbf{Resource type}}& {Val.}  & {\textbf{Bg. 1}} & {\textbf{Bg. 2}} & {\textbf{Bg. 3}} & {\textbf{Bg. 4}} & {\textbf{Bd. 5}} & {\textbf{Bd. 6}} \\
\hline
\multirow{3}{*}{DSP48E} & Predicted & 35 & 69 & 141 & 213 & 285 & 331 \\
 & Measured & 36 & 72 & 144 & 216 & 288 & 360 \\
 & \textbf{Error} & \textbf{-3.2\%} & \textbf{-4.2\%} & \textbf{-2.4\%} & \textbf{-1.2\%} & \textbf{-1.0\%} & \textbf{-0.8\%} \\
\hline
\multirow{3}{*}{DRAM18K} & Predicted & 65 & 87 & 175 & 265 & 354 & 446\\
 & Measured & 64 & 86 & 173 & 259 & 346 & 432 \\
 & \textbf{Error} & \textbf{+1.0\%} & \textbf{+0.8\%} & \textbf{+1.2\%} & \textbf{+2.2\%} & \textbf{+2.4\%} & \textbf{+3.2\%} \\
\hline
\end{tabular}
%\vspace{-0pt}
%\vspace{-0pt}
%\vspace{-2.7em}
\label{tab:val_resource}
\end{table}


%We compared the predicted energy breakdown and latency using the convolution layers of AlexNet and row stationary dataflow using the unit energy adopted in their paper~\cite{eyeriss} and observe a prediction error within \todob{xx} for energy breakdown and \todob{xx} for latency as shown in Table~\ref{fig:val_eyeriss_lat} and Fig.~\ref{fig:val_eyeriss_lat}


\vspace{-1.5em}
\subsection{Evaluation for the \textit{Chip Builder} and \textit{AutoDNNchip}}
\label{subsec:dse}
In this subsection, we evaluate the performance of the proposed \textit{Chip Builder}, which makes use of the time-efficient and accurate \textit{Chip Predictor} to perform an effective two-stage DSE efficiently, and \textit{AutoDNNchip}. Specifically, we study the performance of the resulting DNN accelerators generated and optimized by the \textit{Chip Builder} and \textit{AutoDNNchip}. \ul{First}, we will show experiment results to visualize the \textit{Chip Builder}'s two-stage DSE process; \ul{Second}, we study the performance improvement resulted from the \textit{Chip Builder}'s second-stage IP-pipeline co-optimization in terms of bottleneck blocks' latency and idle cycle reduction; \ul{Finally}, we validate the effectiveness of the \textit{AutoDNNchip} by comparing the performance of the FPGA based accelerators (i.e., the corresponding RTL implementation) generated by the \textit{Chip Builder} with that of state-of-the-art designs under the same conditions. 

%  finally, we go through the compilation and exploration of Chip builder to show we can achieve better performance when we deploy our RTL implementation generated by Chip builder and compare with state-of-the-art design.

% With the help of time-efficient and accurate Chip Predictor, we could enable Chip Builder, through our two-stage design space exploration efficiently. Here, we explore the design space by using architecture-, IP-, dataflow-level co-design for the 2 supported back-ends -- FPGA and ASIC. To validate the effectiveness of Chip Builder, we first visualize the two-stage for the design space exploration process in our Chip Builder; then we evaluate the benefit from our second-stage IP/pipeline co-optimization, by showing the total latency and idle cycles reduction for the detected system bottleneck; finally, we go through the compilation and exploration of Chip builder to show we can achieve better performance when we deploy our RTL implementation generated by Chip builder and compare with state-of-the-art design.
% The results show \todob{xx performance improvement for FPGA and xx performance improvement for ASIC design.}
%Design space exploration for architecture-, IP-, dataflow-level co-design is done for the 2 supported back-ends, FPGA and ASIC with \todob{xx significant performance improvement} through our two-stage optimization process.

\textbf{Evaluation Setup.} In this set of experiments, we consider the application-driven specifications and constraints summarized in Table ~\ref{tab:dse_setting}, where the throughput requirement and power budget are set to meet real-time applications of visual recognition (e.g., image classification and object detection~\cite{faster-rcnn}) on edge devices. For the FPGA accelerator design, we use a state-of-the-art edge device Ultra96 FPGA board ~\cite{ultra96} whose resource budget is fixed. In addition, we 1) use  \textit{Algorithm~\ref{alg:sim}} to perform the accelerator design optimization, and consider 2) the 4 architecture templates shown in Fig.~\ref{fig:arch_temp} in the architecture/dataflow search space and 3) the hyper-parameters in Table~\ref{tab:design_space} for the IP/dataflow design.

% ; \ul{For the ASIC accelerator design}, we set the number of MACs and the total area of the on-chip memories to occupy over 95\% of the chip area~\cite{eyeriss, du2015shidiannao}

% For the two-stage design space exploration approach, we follow the \textit{Algorithm~\ref{fig:alg}} to optimize the accelerator design. For the architecture/dataflow search space for FPGA and ASIC accelerator, we use the 4 architecture templates shown in Fig.~\ref{fig:arch_temp}; for the IP/dataflow design, the search space is shown in Table~\ref{tab:design_space}.

% and the upper bound for each dimension of the search space by Algorithm~\ref{fig:alg}. \todob{show the exact value for each dim?}

\textbf{Visualizing the \textit{Chip Builder}'s Two-stage DSE Process.} For demonstrating the effectiveness of the \textit{Chip Builder}'s two-stage DSE engine, we here show an visualisation of the DSE process, when using \textit{AutoDNNchip} to design an FPGA based accelerator for achieving competitive performance as the award winning state-of-the-art design in ~\cite{zhang2019skynet} given the same target performance specification/constraint, FPGA board, DNN model, and dataset. The FPGA measured energy consumption of both the resulting design from the \textit{AutoDNNchip} and the reported one of ~\cite{zhang2019skynet} are marked in purple in Fig.~\ref{fig:dse_fpga}. The results in Fig.~\ref{fig:dse_fpga} show that 1) the DSE engine of the \textit{Chip Builder} can effectively trim down the design choices and generate an optimized design that can achieve comparable performance (slightly better: 11\% energy savings; \textbf{even better than human design}) with that of the expert-crafted prior art design \cite{zhang2019skynet}, \textbf{showing that with no-human in the loop the \textit{AutoDNNchip} can indeed automatically generate DNN accelerators that achieve optimal target performance}; 2) most of the design choices can be efficiently ruled out by \ul{the 1st stage} of the DSE engine, i.e., the early stage exploration based on the \textit{Chip Predictor}'s coarse-grained analytical performance estimation; and 3) \ul{the 2nd stage} IP-pipeline co-optimization of the \textit{Chip Builder} can effectively boost (up to 41.82\% improvement and an average of 34.5\% improvement) the performance, i.e., throughput of the DNN accelerators here, as compared to that of the  designs resulted from the 1st stage DSE. The final generated design candidates in the HLS code format will be passed to Vivado~\cite{vivado_HLS} for implementation, and we will eliminate the designs that fail the place and route (PnR) as shown in Figure~\ref{fig:dse_fpga}
, and find an optimal design from the remaining ones after PnR. As a reference point, the 1st stage DSE takes about 0.65 ms for each design point and only 0.8 hour for exploring a total of 4.6 million design points when running on an Intel Core i5 CPU with a single thread, thanks to the analytical nature of the \textit{Chip Predictor}.

%\todob{Explanation for the eliminated points: on}


% Our visualization for two-stage DSE process on FPGA is shown in Fig.~\ref{fig:dse_fpga}. Experiment results shown in Fig.~\ref{fig:dse_fpga} samples sufficient points on the design space for each stage (the performance of two purple points denoting our baseline and our optimal one designed by AutoDNNchip is measured on Ultra96 FPGA) to demonstrate we can quickly eliminate most bad design choices and get some possible candidates with potential best performance by the early stage exploration, and significantly improve the overall throughput performance by the 2nd stage IP-pipeline co-optimization.

\textbf{Evaluation of the \textit{Chip Builder}'s 2nd-stage Optimization}. Fig.~\ref{fig:idle_cycles_fpga} summarizes the evaluation experiments for the \textit{Chip Builder}'s 2nd-stage Optimization. As described in Section \ref{sec:dse}, this stage targets an IP-pipeline co-optimization and thus can lead to more balanced pipeline and more efficient resource allocation. From Fig. ~\ref{fig:idle_cycles_fpga}, we can see that the \textit{Chip Builder}'s 2nd-stage optimization can achieve up to 2.4$\times$ idle cycles reduction, when optimizing the design of SkyNet's 6 blocks of SkyNet~\cite{zhang2019skynet} on the Ultra96 FPGA board ~\cite{ultra96}. 



% The benefit for the 2nd stage optimization which targets on IP-pipeline co-optimization is shown Fig.~\ref{fig:idle_cycles_fpga}. Fig.~\ref{fig:idle_cycles_fpga} shows the overall performance gain we observe from the second stages comes from the idle cycles reduction for the system bottleneck IP, resulting in more balanced pipeline stage and more efficient resource allocation for the whole system. The idle cycles are recorded on the same bottleneck IP found by AutoDNNchip for different execution stages (different DNN building blocks) and we can achieve up to 2.4$\times$ idle cycles reduction and 1.7$\times$ total cycles reduction.


% \todob{Experiment result analysis for ASIC}
%  we have the optimized design \todob{describe architecture/IP/dataflow in the same way as Fig.~\ref{fig:toy}, including the ip type, ip tiling, ip interconnection, ip dataflow, intra/inter ip pipeline design}  

% For the \todob{XX} optimization results on ASIC, we have the optimized design \todob{describe architecture/IP/dataflow in the same way as Fig.~\ref{fig:toy}, including the ip type, ip tiling, ip interconnection, ip dataflow, intra/inter ip pipeline design}  

\begin{table}[h!]
% \vspace{-1em}
\caption{The considered application-driven specifications and constraints in the experiments of evaluating the \textit{Chip Builder}'s generated FPGA based DNN accelerators.}
\vspace{-1em}
\def\arraystretch{1.2}
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|}
\hline
{\textbf{Target Back-end}} & {\textbf{Opt. Obj.}} & {\textbf{Th. Req.}} & {\textbf{Power Budget}} & {\textbf{Resource Budget}}\\
\hline
\multirow{2}{*}{\textbf{Ultra96 FPGA}} & \multirow{2}{*}{E, L} & \multirow{2}{*}{20FPS} & \multirow{2}{*}{10W} & {DSP=360, FF=141120}\\
 & &  &  & {LUT=70560, BRAM=432}\\
\hline
% \multirow{2}{*}{\textbf{ASIC}{\todob{??}}} & \multirow{2}{*}{E, L} & \multirow{2}{*}{15FPS} & \multirow{2}{*}{\todob{xxW}} & {Memory Area=\todob{XX} $mm^2$}\\
%  &  &  &  & {\# of MAC units =\todob{XX}}\\
%  \hline
% \vspace{-1em}
\end{tabular}
\vspace{-0pt}


% Experiment setting for design space exploration on the FPGA and ASIC back-end, including optimization object, minimum throughput requirement (FPS) for real-time object detection/image classification, power budget, resource budget.}
% \label{tab:dse_setting}

% onsider the application-driven specifications and constraints summarized in Table ~\ref{tab:dse_setting}, where the throughput requirement and power budget are set to meet real-time applications of visual recognition (e.g., image classification and object detection) on edge devices 
 \label{tab:dse_setting}
%\vspace{-0pt}
%\vspace{-2.7em}
\end{table}


\begin{figure}[h]
\vspace{-1.0em}
    \centerline{\includegraphics[width=1.05\linewidth]{fig/ab_1.pdf}}
    \vspace{-1em}
    \caption{\textbf{Visualizing the energy consumption per image and processing latency of the resulted designs from the \textit{Chip Builder}'s 1st and 2nd stage optimization, when  using \textit{AutoDNNchip} to design an FPGA based accelerator for meeting the  performance of a state-of-the-art design ~\cite{zhang2019skynet} given the same performance specification/constraint, FPGA board, DNN model, and dataset.
    % Design space exploration targeting on SkyNet~\cite{zhang2019skynet} and Ultra96. For the sampled points on the design space, the optimized ones (baseline and the design optimized by AutoDNNchip), the energy/latency is measured on Ultra96 and others are obtained from the prediction of the chip predictor
    }}
    \vspace{-0.5em}
    \label{fig:dse_fpga}
\end{figure}

% For demonstrating the effectiveness of the \textit{Chip Builder}'s two-stage DSE engine, we here show an visualisation of the DSE process, when using \textit{AutoDNNchip} to design an FPGA based accelerator for meeting the  performance of a award winning state-of-the-art design ~\cite{zhang2019skynet} given the same target performance specification/constraint, FPGA board, DNN model, and dataset. 


\begin{figure}[h]

    \centerline{\includegraphics[width=1.1\linewidth]{fig/ab_2.PNG}}
    \vspace{-0.5em}
    \caption{\textbf{The busy and idle cycles of the bottleneck IPs in SkyNet's 6 different blocks, before and after conducting the \textit{Chip Builder}'s 2nd-stage IP-pipeline co-optimization, when using the \textit{AutoDNNchip} to generate designs for the Ultra96 FPGA board with the same target performance as \cite{zhang2019skynet}.}}
    % \vspace{-1.1em}
    \label{fig:idle_cycles_fpga}
\end{figure}


% \begin{figure}[h]
%     \centerline{\includegraphics[width=50mm]{fig/asic_1.pdf}}
%     \vspace{-1em}
%     \caption{\textbf{Design space exploration for ASIC targeting on XX. For the sampled points on the design space, the optimized ones (baseline and the design optimized by AutoDNNchip), the energy/latency is measured on Ultra96 and others are obtained from the prediction of the chip predictor.}\todob{Yang}}
%     \vspace{-1.1em}
%     \label{fig:dse_asic}
% \end{figure}

% \begin{figure}[h]
%     \centerline{\includegraphics[width=50mm]{fig/asic_2.pdf}}
%     \vspace{-1em}
%     \caption{\textbf{ASIC}\todob{By Yang: Reduced idle cycles for the bottleneck IP (simulated) and reduced total latency (measured) when mapping different XXX.}}
%     \vspace{-1.1em}
%     \label{fig:idle_cycles_asic}
% \end{figure}

\textbf{Evaluation of the \textit{AutoDNNchip}'s Generated DNN Accelerators.} 
Fig. \ref{fig:dse_fpga} shows that the DNN accelerator generated by \textit{AutoDNNchip} can outperform the recent award-winning design \cite{zhang2019skynet}. We further conduct another set of experiments to compare the performance of \textit{AutoDNNchip}'s generated DNN accelerators on the Ultra96 FPGA board with that of a mobile CPU (Pixel2 XL~\cite{mobile}), when both 1) adopt the settings in Table~\ref{tab:val_setting}, use the same bit precision and the 10 DNN models in Table~\ref{tab:dnn_sk}, and 2) try to minimize the latency for considering time-critical applications. Note that the DNN mapping to the mobile CPU is optimized using Tensorflow Lite~\cite{tflite}. Fig. \ref{fig:pareto} illustrates the corresponding latency vs. energy efficiency, where the results under the same DNN models are marked with makers of the same shape. We can see that \textit{AutoDNNchip} generated accelerators consistently achieve smaller latency than the baselines under the same DNN model and settings while having similar (<15\% difference) energy efficiency. Specifically, \textit{AutoDNNchip} generated accelerators achieve an average latency reduction of 3.86$\times$ while having slightly better (~10\%) or worse (differs <15\%) energy efficiency, demonstrating the effectiveness of \textit{AutoDNNchip} in generating optimized DNN accelerators.   

% To evaluate the design which is optimized and generated by \textit{Chip Builder} against state-of-the-art design, we further compare our design on the Ultra96 FPGA board with a mobile CPU (Pixel2 XL~\cite{mobile}). We adopt the settings in Table~\ref{tab:val_setting} and map 10 DNN models in Table~\ref{tab:dnn_sk} on our design and the mobile CPU.\todob{the DNN mapping to the mobile CPU is optimized by Tensorflow Lite~\cite{tflite}} Our design has a better latency performance over all 10 DNN models. To be more specific, our design has 3.78$\times$ to 4.69$\times$ latency reduction than the mobile CPU resulting an average of 4.08$\times$ latency reduction with similar energy efficiency. Therefore, for time-critical applications, our design reduces by over 4$\times$ latency under the same energy budget than the mobile CPU. 

%To compare our design which is optimized and generated by \textit{Chip Builder} with state-of-the-art baselines, we adopt the same settings in Table~\ref{tab:val_setting} and map 10 DNN models in Table~\ref{tab:dnn_sk} on our design as well as 2 edge devices including mobile CPU (Pixel2 XL~\cite{mobile}) and edge TPU.
%and the DNN accelerator design on optimized by our tool. 
%Our design has a better latency performance over all 10 DNN models than two baselines. 
%To be more specific, our design has up to 3.89$\times$ latency reduction compared with mobile CPU. 
%In addition, our design achieves up to 4.46$\times$ latency reduction and up to 9.67$\times$ better energy efficiency compared with edge TPU. We can see that our design has a more balanced performance over 10 DNN models than edge TPU because \textit{AutoDNNchip} optimizes the design for various DNN model structure (i.e., short-cut paths and reorganization structures). 
%Considering all 10 DNN model, our design can achieve an average of 3.38$\times$ latency reduction compared with mobile CPU and an average of 2.96$\times$ latency reduction compared with edge TPU. 

 
%We can achieve up to 9.67$\times$ better energy efficiency and 4.46$\times$ latency reduction compared with other baseline edge devices. To be more specific, our design can achieve an average of 1.36$\times$ higher energy efficiency compared with Jetson TX2, 1.82$\times$ latency reduction compared with edge TPU, and 3.33$\times$ latency reduction compared with Pixel2 XL  over 5 DNN models.
%For SkyNet to SK4, which has a network bypass and reorganization layer with some customized operations not well supported on the edge TPU, our design on Ultra96 can outperform edge TPU with 4.20$\times$ latency reduction and 8.90$\times$ better energy efficiency in average; compared with Pixel2 XL , our design on Ultra96 can achieve 3.40$\times$ latency reduction in average.

%For other DNN models w/o a network bypass and reorganization layer, our design can achieve 1.36$\times$ higher energy efficiency compared with Jetson TX2,  1.82$\times$ latency reduction compared with edge TPU, and 3.33$\times$ latency reduction compared with Pixel2 XL  in average.
% \todob{table showing our energy, latency, energy efficiency, utilization, clk frequecy,}
% \todob{Insights about application-driven\\(performance-based) DNN/platform/architecture/IP selection}
% the customized operations is not well supported in Edge TPU for now.
% \todob{Show under what scenarios (DNNs) FPGA/ASIC will win/lose compared with other platforms (performance vs mobile/TPU/GPU on different DNNs) (performance/pipeline opitimization freedom: HLS-based FPGA solution vs ASIC design)}
\begin{figure}[h]
\vspace{-1.1em}
    \centerline{\includegraphics[width=1.1\linewidth]{fig/edge.pdf}}
    \vspace{-1em}
    \caption{\textbf{Processing latency and energy efficiency on Ultra96 FPGA compared with a mobile device (Pixel2 XL ) on 10 compact DNN models}}
    \vspace{-0.5em}
    \label{fig:pareto}
\end{figure}



